Learning RL-Policies for Joint Beamforming Without Exploration: A Batch Constrained Off-Policy Approach

In this work, we consider the problem of network parameter optimization for rate maximization. We frame this as a joint optimization problem of power control, beam forming, and interference cancellation. We consider the setting where multiple Base Stations (BSs) communicate with multiple user equipment (UEs). Because of the exponential computational complexity of brute force search, we instead solve this nonconvex optimization problem using deep reinforcement learning (RL) techniques. Modern communication systems are notorious for their difficulty in exactly modeling their behavior. This limits us in using RL-based algorithms as interaction with the environment is needed for the agent to explore and learn efficiently. Further, it is ill-advised to deploy the algorithm in the real world for exploration and learning because of the high cost of failure. In contrast to the previous RL-based solutions proposed, such as deep-Q network (DQN) based control, we suggest an offline model-based approach. We specifically consider discrete batch-constrained deep Q-learning (BCQ) and show that performance similar to DQN can be achieved with only a fraction of the data without exploring. This maximizes sample efficiency and minimizes risk in deploying a new algorithm to commercial networks. We provide the entire project resource, including code and data, at the following link: https://github.com/Heasung-Kim/ safe-rl-deployment-for-5g.

==> commands.tex <==
\usepackage{algorithmic, algorithm}
\usepackage{mathtools}
\newcommand{\D}{\mathbb{D}}
\newcommand{\Wtwo}{\mathcal{W}_2}
\DeclareGraphicsRule{.eps}{pdf}{.pdf}{`epstopdf #1}
\pdfcompresslevel=9

\newcommand{\Expect}{\mathbb{E}}
\newcommand{\ud}{\,\mathrm{d}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zero}{\mathbf{0}}

\newcommand{\op}[1]{\operatorname{#1}}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\trace}{\op{Tr}}
\newcommand{\Tan}{\op{Tan}}
\renewcommand{\tilde}{\widetilde}
\newcommand{\cvx}{\mathtt{CVX}}
\newcommand{\icvx}{\mathtt{ICNN}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\prim}{\op{primal}}
\newcommand{\dual}{\op{dual}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\argmax}{\mathop{\operatorname{argmax}}}
\newcommand{\argmin}{\mathop{\operatorname{argmin}}}

\newcommand{\W}{\mathds{W}}

\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}

\newcommand{\newP}[1]{\paragraph{#1.}}
\newcommand{\RM}{\text{RM}}
\newcommand{\KO}{\text{KO}}

\usepackage{comment}
% ------------ THEOREMS

\usepackage{thmtools}

\declaretheorem[numberwithin=section]{theorem}
\declaretheorem[sibling=theorem]{lemma}
\declaretheorem[sibling=theorem]{proposition}
\declaretheorem[sibling=theorem]{corollary}
\declaretheorem[sibling=theorem]{remark}
\declaretheorem[sibling=theorem]{definition}
\declaretheorem[sibling=theorem]{example}
\declaretheorem{assumption}


\usepackage{prettyref,xspace}
\usepackage{tikz}

%\usepackage{authblk}


\newcommand{\xmark}{\text{\ding{55}}}

\newrefformat{cond}{Condition~\ref{#1}}
\newrefformat{eq}{(\ref{#1})}
\newrefformat{thm}{Theorem~\ref{#1}}
\newrefformat{th}{Theorem~\ref{#1}}
\newrefformat{chap}{Chapter~\ref{#1}}
\newrefformat{sec}{Section~\ref{#1}}
\newrefformat{algo}{Algorithm~\ref{#1}}
\newrefformat{fig}{Figure~\ref{#1}}
\newrefformat{tab}{Table~\ref{#1}}
\newrefformat{rmk}{Remark~\ref{#1}}
\newrefformat{clm}{Claim~\ref{#1}}
\newrefformat{def}{Definition~\ref{#1}}
\newrefformat{cor}{Corollary~\ref{#1}}
\newrefformat{lmm}{Lemma~\ref{#1}}
\newrefformat{prop}{Proposition~\ref{#1}}
\newrefformat{pr}{Proposition~\ref{#1}}
\newrefformat{app}{Appendix~\ref{#1}}
\newrefformat{prob}{Problem~\ref{#1}}
\newrefformat{ques}{Question~\ref{#1}}
\newrefformat{note}{Note~\ref{#1}}
\newrefformat{assump}{Assumption~\ref{#1}}
\newrefformat{issue}{Issue ~\ref{#1}}
\newrefformat{fix}{Fix ~\ref{#1}}

            


\newcommand{\red}{\color{red}}
\newcommand{\blue}{\color{blue}}
\newcommand{\nb}[1]{{\sf\blue#1}}
\newcommand{\nbr}[1]{{\sf\red[#1]}}
\newcommand{\Mod}[1]{\ (\text{mod}\ #1)}

\newcommand{\torus}{\mathbb{T}}
\newcommand{\diverge}{\to\infty}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\naturals}{\mathbb{N}}
\newcommand{\integers}{\mathbb{Z}}
%\newcommand{\Expect}{\mathbb{E}}
\newcommand{\expect}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\prob}[1]{\mathbb{P}\left(#1\right)}
\newcommand{\pprob}[1]{\mathbb{P}[#1]}
\newcommand{\simplex}{\Delta_n}
\newcommand{\feps}{f_\varepsilon}
\newcommand{\suf}[1]{^{(#1)}}




\newcommand{\inner}[2]{\langle {#1}, {#2}  \rangle}
\newcommand{\realpart}{\mathrm{Re}}
\newcommand{\impart}{\mathrm{Im}}


\newcommand{\ty}{\tilde{y}}
\newcommand{\hTheta}{\hat{\Theta}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
%\newcommand{\calC}{\mathcal{C}}
%\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
%\newcommand{\calF}{\mathcal{F}}
%\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
%\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
%\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
%\newcommand{\calX}{\mathcal{X}}
%\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}



%% All hat symbols

\newcommand{\hA}{\hat{A}}
\newcommand{\hB}{\hat{B}}
\newcommand{\hC}{\hat{C}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hG}{\hat{G}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hI}{\hat{I}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hK}{\hat{K}}
\newcommand{\hL}{\hat{L}}
\newcommand{\hM}{\hat{M}}
\newcommand{\hN}{\hat{N}}
\newcommand{\hO}{\hat{O}}
\newcommand{\hP}{\hat{P}}
\newcommand{\hQ}{\hat{Q}}
\newcommand{\hR}{\hat{R}}
\newcommand{\hS}{\hat{S}}
\newcommand{\hT}{\hat{T}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hV}{\hat{V}}
\newcommand{\hW}{\hat{W}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hY}{\hat{Y}}
\newcommand{\hZ}{\hat{Z}}


\newcommand{\ha}{\hat{a}}
\newcommand{\hb}{\hat{b}}
\newcommand{\hc}{\hat{c}}
\newcommand{\hd}{\hat{d}}
\newcommand{\he}{\hat{e}}
\newcommand{\hf}{\hat{f}}
\newcommand{\hg}{\hat{g}}
\newcommand{\hh}{\hat{h}}
\newcommand{\hi}{\hat{i}}
\newcommand{\hj}{\hat{j}}
\newcommand{\hk}{\hat{k}}
\newcommand{\hl}{\hat{l}}
%\newcommand{\hm}{\hat{m}}
\newcommand{\hn}{\hat{n}}
\newcommand{\ho}{\hat{o}}
\newcommand{\hp}{\hat{p}}
\newcommand{\hq}{\hat{q}}
\newcommand{\hr}{\hat{r}}
\newcommand{\hs}{\hat{s}}
%\newcommand{\ht}{\hat{t}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hv}{\hat{v}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hz}{\hat{z}}

%% All bold symbols
\newcommand{\vect}[1]{\boldsymbol{#1}}

\newcommand{\ba}{\vect{a}}
\newcommand{\bb}{\vect{b}}
\newcommand{\bc}{\vect{c}}
\newcommand{\bd}{\vect{d}}
\newcommand{\be}{\vect{e}}
%\newcommand{\bf}{\textbf{f}}
\newcommand{\bfa}{\vect{f}}
\newcommand{\bg}{\vect{g}}
\newcommand{\bh}{\vect{h}}
\newcommand{\bi}{\vect{i}}
\newcommand{\bj}{\vect{j}}
\newcommand{\bk}{\vect{k}}
\newcommand{\bl}{\vect{l}}
\newcommand{\bma}{\vect{m}}
%\newcommand{\bm}{\textbf{m}}
\newcommand{\bn}{\vect{n}}
\newcommand{\bo}{\vect{o}}
\newcommand{\bp}{\vect{p}}
\newcommand{\bq}{\vect{q}}
\newcommand{\br}{\vect{r}}
\newcommand{\bs}{\vect{s}}
\newcommand{\bt}{\vect{t}}
\newcommand{\bu}{\vect{u}}
\newcommand{\bv}{\vect{v}}
\newcommand{\bw}{\vect{w}}
\newcommand{\bx}{\vect{x}}
\newcommand{\by}{\vect{y}}
\newcommand{\bz}{\vect{z}}


\newcommand{\beps}{\bm{\varepsilon}}
\newcommand{\bGamma}{\vect{\Gamma}}
\newcommand{\bmu}{\vect{P}}
\newcommand{\balpha}{\vect{\alpha}}
\newcommand{\bbeta}{\vect{\beta}}


\newcommand{\bA}{\vect{A}}
\newcommand{\bB}{\vect{B}}
\newcommand{\bC}{\vect{C}}
\newcommand{\bD}{\vect{D}}
\newcommand{\bE}{\vect{E}}
%\newcommand{\bF}{\textbf{F}}
\newcommand{\bG}{\vect{G}}
\newcommand{\bH}{\vect{H}}
\newcommand{\bI}{\vect{I}}
\newcommand{\bJ}{\vect{J}}
\newcommand{\bK}{\vect{K}}
\newcommand{\bL}{\vect{L}}
\newcommand{\bM}{\vect{M}}
\newcommand{\bN}{\vect{N}}
\newcommand{\bO}{\vect{O}}
\newcommand{\bP}{\vect{P}}
\newcommand{\bQ}{\vect{Q}}
\newcommand{\bR}{\vect{R}}
\newcommand{\bS}{\vect{S}}
\newcommand{\bT}{\vect{T}}
\newcommand{\bU}{\vect{U}}
\newcommand{\bV}{\vect{V}}
\newcommand{\bW}{\vect{W}}
\newcommand{\bX}{\vect{X}}
\newcommand{\bY}{\vect{Y}}
\newcommand{\bZ}{\vect{Z}}


%%  Addition, norm, absolute, compact summation
\newcommand{\mat}[2]{\reals^{#1 \times #2}}
\newcommand{\abs}[1]{\left|{#1} \right|}
%\newcommand{\norm}[1]{\left \|#1\right \|}
\newcommand{\normsqr}[1]{\|#1\|^2}
\newcommand{\soft}{\mathrm{softmax}}
\newcommand{\derv}[2]{\frac{\partial{#1}}{\partial {#2}}}
\newcommand{\tilh}{\tilde{h}}
\newcommand{\diag}[1]{\mathrm{diag}(#1)}
\newcommand{\add}[3]{\sum_{#1=#2}^{#3}}
\newcommand{\compsum}[2]{\sum_{#1 \in [#2]}}


\newcommand{\unif}{\mathrm{Unif}}
\newcommand{\valid}{\mathrm{valid}}

%% Tailored to my definitions mathrm things

\newcommand{\even}{\ \mathrm{even}}
\newcommand{\odd}{\ \mathrm{odd}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\disc}{\mathrm{disc}}
%\newcommand{\argmin}{\mathrm{arg}\min}
\newcommand{\binary}{\{0,1\}}
\newcommand{\sym}{\mathrm{sym}}
\newcommand{\lse}{\mathrm{LSE}}
\newcommand{\define}{\triangleq}




%% parenthesis
\newcommand{\pth}[1]{\left( #1 \right)}
\newcommand{\qth}[1]{\left[ #1 \right]}
\newcommand{\sth}[1]{\left\{ #1 \right\}}
\newcommand{\floor}[1]{{\left\lfloor {#1} \right \rfloor}}
\newcommand{\ceil}[1]{{\left\lceil {#1} \right \rceil}}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\ie}{i.e.\xspace}
\newcommand{\iid}{i.i.d.\xspace}
\newcommand{\dark}[1]{\textbf{#1}}
\newcommand{\samplex}[1]{x^{({#1})}}
\newcommand{\sampley}[1]{y^{({#1})}}

\newcommand{\Id}{\mathrm{Id}}
\mathchardef\mhyphen="2D 

\newcommand{\nreed}{\mathrm{NPC}}
\newcommand{\reed}{\mathrm{RM}} %\mathcal{R}\mathcal{M}}
\definecolor{MyGreen1}{RGB}{20,180,40}

\newcommand*{\texthash}[0]{\#}
\usepackage{siunitx}
